Bounds on the Capacity of the Multiple Access Diamond Channel with Cooperating Base-Stations

A diamond network is considered in which the central processor is connected, via backhaul noiseless links, to multiple conferencing base stations, which communicate with a single user over a multiple access channel. We propose coding techniques along with lower and upper bounds on the capacity. Our achievability scheme uses a common cloud coding strategy based on the technique proposed by Wand, Wigger, and Zaidi (2018) and extends it beyond two relays. Our upper bounds generalize the method proposed by Bidokhti and Kramer for the two relay diamond network without cooperation (2016) and lead to new bounds for the multiple relay setting. Specializing our upper bounds for the two relay scenario (with cooperation), we provide new bounds and improve state-of-the-art.

==> sections/2bs_1mu/upper_bounds/dpi_cran_conf_proof.tex <==
First, we use the chain rule to expand $ I(\rv{X}_1^n ;\rv{X}_2^n,\rv{W}_2|\rv{W}_{12},\rv{W}_{21}) $ in the two following different ways:
\begin{align}
I(\rv{X}_1^n;\rv{X}_2^n,\rv{W}_2|\rv{W}_{12},\rv{W}_{21}) 
&= I(\rv{X}_1^n;\rv{W}_2|\rv{W}_{12},\rv{W}_{21})  + I(\rv{X}_1^n;\rv{X}_2^n|\rv{W}_2,\rv{W}_{12},\rv{W}_{21})  =  I(\rv{X}_1^n;\rv{W}_2|\rv{W}_{12},\rv{W}_{21}) \\
&= I(\rv{X}_1^n;\rv{X}_2^n|\rv{W}_{12},\rv{W}_{21})  
+ I(\rv{X}_1^n;\rv{W}_2|\rv{X}_2^n,\rv{W}_{12},\rv{W}_{21}) 
\geq I(\rv{X}_1^n;\rv{X}_2^n|\rv{W}_{12},\rv{W}_{21}) .
\end{align}
In a very similar method, we will use again the chain rule to expand $ I(\rv{W}_1,\rv{X}_1^n;\rv{W}_2|\rv{W}_{12},\rv{W}_{21})  $ in the following fashion:
\begin{align}
I(\rv{W}_1,\rv{X}_1^n;\rv{W}_2|\rv{W}_{12},\rv{W}_{21})
&= I(\rv{W}_1;\rv{W}_2|\rv{W}_{12},\rv{W}_{21}) + I(\rv{X}_1^n;\rv{W}_2|\rv{W}_1,\rv{W}_{12},\rv{W}_{21}) = I(\rv{W}_1;\rv{W}_2|\rv{W}_{12},\rv{W}_{21}) \\
&= I(\rv{X}_1^n;\rv{W}_2|\rv{W}_{12},\rv{W}_{21}) +
I(\rv{W}_1;\rv{W}_2|\rv{X}_1^n,\rv{W}_{12},\rv{W}_{21}) 
\geq I(\rv{X}_1^n;\rv{W}_2|\rv{W}_{12},\rv{W}_{21}).
\end{align}
Combining those inequalities we obtain the following Data Processing Inequality:
\begin{equation}
I(\rv{X}_1^n;\rv{X}_2^n|\rv{W}_{12},\rv{W}_{21})   \leq I(\rv{W}_1;\rv{W}_2|\rv{W}_{12},\rv{W}_{21}) .
\end{equation}
We proceed to derive an upper bound on $ I(\rv{W}_1;\rv{W}_2|\rv{W}_{12},\rv{W}_{21}) $. Consider the subsequent list of inequalities:
\begin{align}
I(\rv{W}_1;\rv{W}_2|\rv{W}_{12},\rv{W}_{21}) 
&= H(\rv{W}_1|\rv{W}_{12},\rv{W}_{21})  - H(\rv{W}_1|\rv{W}_2,\rv{W}_{12},\rv{W}_{21}) \\
&= H(\rv{W}_1|\rv{W}_{12},\rv{W}_{21})  - H(\rv{W}_1|\rv{W}_2,\rv{W}_{21}) \\
&\leq H(\rv{W}_1|\rv{W}_{21})  - H(\rv{W}_1|\rv{W}_2,\rv{W}_{21}) \\
& = I(\rv{W}_1;\rv{W}_2|\rv{W}_{21}) \\
&= H(\rv{W}_2|\rv{W}_{12})-  H(\rv{W}_2|\rv{W}_1,\rv{W}_{21}) \\
&= H(\rv{W}_2|\rv{W}_{21})-  H(\rv{W}_2|\rv{W}_1) \\
&\leq H(\rv{W}_2)-  H(\rv{W}_2|\rv{W}_1) \\
&= I(\rv{W}_1;\rv{W}_2).
\end{align}
This completes the proof of the lemma.

==> sections/2bs_1mu/upper_bounds/multiletter_upper_bound_proof.tex <==

By Fano's inequality \cite[Theorem 2.10.1]{Cover2006},
\begin{align}
	nR &= H(\rv{M}) \\
	&= I(\rv{M};\hat{\rv{M}}) + H(\rv{M}|\hat{\rv{M}}) \\
	&\leq I(\rv{M};\rv{Y}^n) + n \epsilon_n,
\end{align}
where $ \epsilon_n $ tends to zero as $ n \rightarrow \infty $.  Further, applying \acrfull{dpi} \cite{Cover2006} on the Markov chain $ \rv{M} \rightarrow (\rv{W}_1,\rv{W}_2) \rightarrow \rv{Y} $, we obtain
\begin{align}
	I(\rv{M};\rv{Y}^n)
	&\leq I(\rv{W}_1,\rv{W}_2;\rv{Y}^n) \\
	&=  H(\rv{W}_1,\rv{W}_2 ) - H(\rv{W}_1,\rv{W}_2|\rv{Y}^n) \\
	&\eqann{\leq}{a} H(\rv{W}_1,\rv{W}_2) \\
	&= H(\rv{W}_1) + H(\rv{W}_2)  - I(\rv{W}_1;\rv{W}_2) \\
	&\leq nC_{1} + nC_{2} - I(\rv{W}_1;\rv{W}_2) ,
\end{align}
where \eqannref{a} follows from non-negativity of entropy. We proceed to find a lower bound on $ I(\rv{S}_1^n;\rv{S}_2^n) $. We give two lower bounds. 
Note that since $ \rv{V}_{1,k} = g_1(\rv{S}_1^n, \rv{V}_{2}^{k-1}) $ and $ \rv{V}_{2,k} = g_2(\rv{S}_2^n, \rv{V}_{1}^{k-1}) $, we have
\begin{align}
	I(\rv{S}_1^n;\rv{S}_2^n) 
	&= H(\rv{S}_1^n) - H(\rv{S}_1^n|\rv{S}_2^n) \\
	&= H(\rv{S}_1^n) - H(\rv{S}_1^n|\rv{S}_2^n, \rv{V}_{2,1}) \\
	&= I(\rv{S}_1^n;\rv{S}_2^n, \rv{V}_{2,1}) \\
	&= H(\rv{S}_2^n, \rv{V}_{2,1}) - H(\rv{S}_2^n, \rv{V}_{2,1}|\rv{S}_1^n) \\
	&= H(\rv{S}_2^n, \rv{V}_{2,1}) - H(\rv{S}_2^n, \rv{V}_{2,1}|\rv{S}_1^n, \rv{V}_{1,1}) \\
	&= I(\rv{S}_1^n, \rv{V}_{1,1};\rv{S}_2^n, \rv{V}_{2,1}) \\
	&= H(\rv{S}_1^n, \rv{V}_{1,1})  -  H(\rv{S}_1^n, \rv{V}_{1,1}|\rv{S}_2^n, \rv{V}_{2,1}) \\
	&= H(\rv{S}_1^n, \rv{V}_{1,1})  -  H( \rv{V}_{1,1}|\rv{S}_2^n, \rv{V}_{2,1}) -H(\rv{S}_1^n,|\rv{S}_2^n, \rv{V}_{2,1},\rv{V}_{1,1})\\
	&= H(\rv{S}_1^n, \rv{V}_{1,1})  -  H( \rv{V}_{1,1}|\rv{S}_2^n, \rv{V}_{2,1}) -H(\rv{S}_1^n,|\rv{S}_2^n, \rv{V}_{2}^2,\rv{V}_{1,1})\\
\end{align}

The first one incorporates \autoref{lemma:dpi_cran_conf}. Using the inequality in \eqref{eq:dpi_cran_conf}, we obtain.
\begin{equation}
	nR \leq nC_1+nC_2 - I(\rv{X}_1^n;\rv{X}_2^n|\rv{W}_{12},\rv{W}_{21}).
\end{equation}
We can also develop a different lower bound on $ I(\rv{W}_1;\rv{W}_2) $ as follows. Consider the mutual information between the channel input sequences,
\begin{align}
	I(\rv{X}_1^n;\rv{X}_2^n)
	&\eqann{\leq}{a}  I(\rv{W}_1,\rv{W}_{12};\rv{W}_2,\rv{W}_{21}) \\
	&= H(\rv{W}_1,\rv{W}_{12}) + H(\rv{W}_2,\rv{W}_{21}) - H(\rv{W}_1,\rv{W}_{12},\rv{W}_{21},\rv{W}_{2}) \\
	&= H(\rv{W}_1) + H(\rv{W}_{12}|\rv{W}_1) + H(\rv{W}_2) + H(\rv{W}_{21}|\rv{W}_2)   - H(\rv{W}_1,\rv{W}_{2}) - H(\rv{W}_{12},\rv{W}_{21}|\rv{W}_1,\rv{W}_{2}) \\
	&\eqann{=}{b} H(\rv{W}_1) + H(\rv{W}_{12}|\rv{W}_1) + H(\rv{W}_2) + H(\rv{W}_{21}|\rv{W}_2)   - H(\rv{W}_1,\rv{W}_{2}) \\
	&\leq H(\rv{W}_1) + H(\rv{W}_{12}) + H(\rv{W}_2) + H(\rv{W}_{21})   - H(\rv{W}_1,\rv{W}_{2})  \\
	&\leq I(\rv{W}_1;\rv{W}_2) + nC_{12} +  nC_{21}
\end{align}
where \eqannref{a}  is due to \acrshort{dpi} applied on the Markov chain $ \rv{X}_1^n \rightarrow (\rv{W}_1,\rv{W}_{12}) \rightarrow (\rv{W}_2,\rv{W}_{21}) \rightarrow \rv{X}_2^n $. Equality in \eqannref{b} follows since $ (\rv{W}_{12},\rv{W}_{21}) $ is a deterministic function of $ (\rv{W}_1,\rv{W}_2) $. Therefore,   
\begin{equation}
	nR \leq n(C_{1}+C_{2}+C_{12}+C_{21})- I(\rv{X}_1^n,\rv{X}_2^n) + n\epsilon_n.
\end{equation}
Considering the Markov chain $ \rv{M} \rightarrow (\rv{W}_1,\rv{W}_2) \rightarrow  (\rv{X}_1^n,\rv{W}_2,\rv{W}_{21}) \rightarrow (\rv{X}_1^n,\rv{X}_2^n) \rightarrow \rv{Y}^n $, following bound is obtained
\begin{align*}
	I(\rv{M};\rv{Y}^n)
	&\leq I(\rv{W}_1,\rv{W}_{2};\rv{Y}^n) \\
	&= I(\rv{W}_1;\rv{Y}^n|\rv{W}_{2}) + I(\rv{W}_{2};\rv{Y}^n) \\
	&\leq I(\rv{W}_1;\rv{W}_{12},\rv{W}_{21},\rv{Y}^n|\rv{W}_{2}) + H(\rv{W}_{2}) \\
	&\leq I(\rv{W}_1;\rv{Y}^n|\rv{W}_{12},\rv{W}_{21},\rv{W}_{2}) +  I(\rv{W}_1;\rv{W}_{12},\rv{W}_{21}|\rv{W}_{2}) + n C_2 \\
	&\eqann{\leq}{a} I(\rv{X}_1^n;\rv{Y}^n|\rv{W}_{12},\rv{W}_{21},\rv{X}_{2}^n) +  I(\rv{W}_1;\rv{W}_{12}|\rv{W}_{2}) + I(\rv{W}_1;\rv{W}_{21}|\rv{W}_{12},\rv{W}_{2}) + n C_2 \\
	&= I(\rv{X}_1^n;\rv{Y}^n|\rv{W}_{12},\rv{W}_{21},\rv{X}_{2}^n) +  H(\rv{W}_{21}|\rv{W}_{2}) + n C_2 \\
	&\leq I(\rv{X}_1^n;\rv{Y}^n|\rv{W}_{12},\rv{W}_{21},\rv{X}_{2}^n) +  H(\rv{W}_{21}) + n C_2 \\
	&\leq I(\rv{X}_1^n;\rv{Y}^n|\rv{W}_{12},\rv{W}_{21},\rv{X}_{2}^n) +  n C_{21} + n C_2 ,
\end{align*}
where equality in \eqannref{a} follows since $ \rv{X}_1^n $ and $ \rv{X}_2^n $ are determined by $ (\rv{W}_1,\rv{W}_{12}) $ and respectively $ (\rv{W}_2,\rv{W}_{21}) $.
Thus,
\begin{equation}
	nR \leq n C_2 + n C_{21} +  I(\rv{X}_1^n;\rv{Y}^n|\rv{W}_{12},\rv{W}_{21},\rv{X}_{2}^n) .
\end{equation}
In similar fashion,
\begin{equation}
	nR \leq n C_1 + n C_{12} +  I(\rv{X}_2^n;\rv{Y}^n|\rv{W}_{12},\rv{W}_{21},\rv{X}_{1}^n) .
\end{equation}
Further note that 
\begin{align}
	I(\rv{W}_{1},\rv{W}_{2};\rv{Y}^n)
	&= I(\rv{W}_{1},\rv{W}_{2},\rv{W}_{12}, \rv{W}_{21};\rv{Y}^n) \\
	&= I(\rv{W}_{1},\rv{W}_{2};\rv{Y}^n|\rv{W}_{12}, \rv{W}_{21}) +  I(\rv{W}_{12}, \rv{W}_{21};\rv{Y}^n) \\
	&= I(\rv{X}_{1}^n,\rv{X}_{2}^n;\rv{Y}^n|\rv{W}_{12}, \rv{W}_{21}) +  H(\rv{W}_{12}, \rv{W}_{21})-H(\rv{W}_{12}, \rv{W}_{21}|\rv{Y}^n) \\
	&\leq  I(\rv{X}_{1}^n,\rv{X}_{2}^n;\rv{Y}^n|\rv{W}_{12}, \rv{W}_{21}) +  H(\rv{W}_{12}, \rv{W}_{21}) \\
	&=  I(\rv{X}_{1}^n,\rv{X}_{2}^n;\rv{Y}^n|\rv{W}_{12}, \rv{W}_{21}) +  H(\rv{W}_{12})+H(\rv{W}_{21})-I(\rv{W}_{12}, \rv{W}_{21}) \\
	&\leq  I(\rv{X}_{1}^n,\rv{X}_{2}^n;\rv{Y}^n|\rv{W}_{12}, \rv{W}_{21}) +  nC_{12}+nC_{21}.
\end{align}
Thus, 
\begin{equation}
	R \leq C_{12}+C_{21} + \frac{1}{n}  I(\rv{X}_{1}^n,\rv{X}_{2}^n;\rv{Y}^n|\rv{W}_{12}, \rv{W}_{21}).
\end{equation}


==> sections/2bs_1mu/upper_bounds/upper3_bound_proof.tex <==

By Fano's inequality $ H(\rv{M}|\hat{\rv{M}}) \leq n \epsilon_n $ where $ \epsilon_n $ tends to zero as $ n \rightarrow \infty $. Therefore,
\begin{equation}
	nR
	= H(\rv{M}) - H(\rv{M}|\hat{\rv{M}}) + H(\rv{M}|\hat{\rv{M}}) \\
	\leq I(\rv{M};\hat{\rv{M}}) + n\epsilon_n \leq I(\rv{W}_1,\rv{W}_2;\rv{Y}^n) + n\epsilon_n.
\end{equation}
The mutual information term $ I(\rv{W}_1,\rv{W}_2;\rv{Y}^n) $ can be bounded from above in a variety of methods.
\begin{align}
	I(\rv{W}_1,\rv{W}_2;\rv{Y}^n) 
	&= I(\rv{W}_1;\rv{Y}^n|\rv{W}_2) + I(\rv{W}_2;\rv{Y}^n) \\
	&\leq I(\rv{W}_1;\rv{W}_{12},\rv{W}_{21},\rv{Y}^n|\rv{W}_2) + H(\rv{W}_2)  \\
	&\leq I(\rv{W}_1;\rv{Y}^n|\rv{W}_{12},\rv{W}_{21},\rv{W}_2) + I(\rv{W}_1;\rv{W}_{12},\rv{W}_{21}|\rv{W}_2)+nC_2. \label{eq:upper_bound4_proof_term2}
\end{align}
The first term in \eqref{eq:upper_bound4_proof_term2} satisfies
\begin{align*}
	I(\rv{W}_1;\rv{Y}^n|\rv{W}_{12},\rv{W}_{21},\rv{W}_2)
	&= \sum_{i=1}^n I(\rv{W}_1;\rv{Y}_i|\rv{W}_{12},\rv{W}_{21},\rv{W}_2,\rv{Y}^{i-1}) \\
	&= \sum_{i=1}^n H(\rv{Y}_i|\rv{W}_{12},\rv{W}_{21},\rv{W}_2,\rv{Y}^{i-1}) - H(\rv{Y}_i|\rv{W}_1,\rv{W}_{12},\rv{W}_{21},\rv{W}_2,\rv{Y}^{i-1}) \\
	&= \sum_{i=1}^n H(\rv{Y}_i|\rv{W}_{12},\rv{W}_{21},\rv{W}_2,\rv{X}_{2i},\rv{Y}^{i-1}) - H(\rv{Y}_i|\rv{W}_1,\rv{W}_{12},\rv{W}_{21},\rv{W}_2,\rv{X}_{1i},\rv{X}_{2i},\rv{Y}^{i-1}) \\
	&\leq \sum_{i=1}^n H(\rv{Y}_i|\rv{W}_{12},\rv{W}_{21},\rv{X}_{2i},\rv{Y}^{i-1}) - H(\rv{Y}_i|\rv{W}_{12},\rv{W}_{21},\rv{X}_{1i},\rv{X}_{2i},\rv{Y}^{i-1}) \\
	&= \sum_{i=1}^n I(\rv{X}_{1i};\rv{Y}_i|\rv{W}_{12},\rv{W}_{21},\rv{X}_{2i},\rv{Y}^{i-1}).
\end{align*}
Identify the auxiliary random variable $ \tilde{\rv{U}}_i \triangleq (\rv{W}_{12},\rv{W}_{21},\rv{Y}^{i-1}) $ and let the time-sharing random variable $ \rv{Q} $ be uniformly distribute over $ [1:n] $ and independent of $ (\rv{M},\rv{W}_1,\rv{W}_2,\rv{W}_{12},\rv{W}_{21},\rv{X}_1^n,\rv{X}_2^n.\rv{Y}^n) $. It follows that
\begin{align}
	I(\rv{W}_1;\rv{Y}^n|\rv{W}_{12},\rv{W}_{21},\rv{W}_2)
	&\leq \sum_{i=1}^n I(\rv{X}_{1i};\rv{Y}_i|\tilde{\rv{U}}_{i},\rv{X}_{2i}) \\
	&= n I(\rv{X}_{1\rv{Q}};\rv{Y}_\rv{Q}|\tilde{\rv{U}}_{\rv{Q}},\rv{X}_{2\rv{Q}}, \rv{Q}).
\end{align}
Now consider the second term in \eqref{eq:upper_bound4_proof_term2}
\begin{align}
	I(\rv{W}_1;\rv{W}_{12},\rv{W}_{21}|\rv{W}_2) 
	&= I(\rv{W}_1;\rv{W}_{12}|\rv{W}_2)  + I(\rv{W}_1;\rv{W}_{21}|\rv{W}_{12},\rv{W}_2) \\
	&= H(\rv{W}_{21}|\rv{W}_{12},\rv{W}_2) \\
	&\leq H(\rv{W}_{21}) \\
	&\leq nC_{21}.
\end{align}
Therefore
\begin{equation}
	\frac{1}{n}  I(\rv{W}_1,\rv{W}_2;\rv{Y}^n)
	\leq C_2+C_{21} + I(\rv{X}_{1\rv{Q}};\rv{Y}_\rv{Q}|\tilde{\rv{U}}_{\rv{Q}},\rv{X}_{2\rv{Q}}, \rv{Q}).
\end{equation}
By symmetric construction, in a very similar method one can also show that
\begin{equation}
	\frac{1}{n}  I(\rv{W}_1,\rv{W}_2;\rv{Y}^n) 
	\leq C_1+C_{12} + I(\rv{X}_{2\rv{Q}};\rv{Y}_\rv{Q}|\tilde{\rv{U}}_{\rv{Q}},\rv{X}_{1\rv{Q}}, \rv{Q}).
\end{equation}
Moreover,
\begin{align}
	I(\rv{W}_1,\rv{W}_2;\rv{Y}^n)  
	&\leq I(\rv{W}_1,\rv{W}_2;\rv{W}_{12},\rv{W}_{21},\rv{Y}^n) \\
	&= I(\rv{W}_1,\rv{W}_2;\rv{Y}^n|\rv{W}_{12},\rv{W}_{21}) + I(\rv{W}_1,\rv{W}_2;\rv{W}_{12},\rv{W}_{21}). \label{eq:upper_bound34_proof_term}
\end{align}
The first term in \eqref{eq:upper_bound34_proof_term} satisfies
\begin{align*}
	I(\rv{W}_1,\rv{W}_2;\rv{Y}^n|\rv{W}_{12},\rv{W}_{21})
	&= \sum_{i=1}^n I(\rv{W}_1,\rv{W}_2;\rv{Y}_i|\rv{W}_{12},\rv{W}_{21},\rv{Y}^{i-1}) \\
	&= \sum_{i=1}^n I(\rv{W}_1,\rv{W}_2,\rv{X}_{1i},\rv{X}_{2i};\rv{Y}_i|\tilde{\rv{U}}_{i}) \\
	&= \sum_{i=1}^n I(\rv{X}_{1i},\rv{X}_{2i};\rv{Y}_i|\tilde{\rv{U}}_{i}) \\
	&= n  I(\rv{X}_{1\rv{Q}},\rv{X}_{2\rv{Q} };\rv{Y}_\rv{Q}|\tilde{\rv{U}}_{\rv{Q}},\rv{Q})  .
\end{align*}
The second term in \eqref{eq:upper_bound34_proof_term} gives
\begin{align}
	I(\rv{W}_1,\rv{W}_2;\rv{W}_{12},\rv{W}_{21})
	&= H(\rv{W}_{12},\rv{W}_{21}) \\
	&\leq H(\rv{W}_{12}) + H(\rv{W}_{21}) \\
	&\leq n(C_{12}+C_{21}).
\end{align}
Thus, we have the following additional constraint on the achievable rate,
\begin{equation*}
	\frac{1}{n} I(\rv{W}_1,\rv{W}_2;\rv{Y}^n)
	\leq I(\rv{X}_{1\rv{Q}},\rv{X}_{2\rv{Q} };\rv{Y}_\rv{Q}|\tilde{\rv{U}}_{\rv{Q}},\rv{Q})  + C_{12}+C_{21}.
\end{equation*}
Next, utilizing \autoref{lemma:dpi_cran_conf}, we obtain the following list of inequalities
\begin{align}
	I(\rv{W}_1,\rv{W}_2;\rv{Y}^n)
	&\leq H(\rv{W}_1,\rv{W}_2) \\
	&= H(\rv{W}_1) + H(\rv{W}_2) -  I(\rv{W}_1;\rv{W}_2) \\
	&\leq n C_1 + nC_2-  I(\rv{W}_1;\rv{W}_2) \\
	&\leq n C_1 + nC_2-  I(\rv{X}_1^n;\rv{X}_2^n|\rv{W}_{12},\rv{W}_{21}) . \label{eq:upper_bound_proof55}
\end{align}
Consider the last term in \eqref{eq:upper_bound_proof55}.
\begin{align}
	I(\rv{X}_1^n;\rv{X}_2^n|\rv{W}_{12},\rv{W}_{21}) 
	& = I(\rv{X}_1^n;\rv{X}_2^n,\rv{Y}^n|\rv{W}_{12},\rv{W}_{21})  - I(\rv{X}_1^n;\rv{Y}^n|\rv{W}_{12},\rv{W}_{21},\rv{X}_2^n) \\
	& = I(\rv{X}_1^n;\rv{Y}^n|\rv{W}_{12},\rv{W}_{21}) + I(\rv{X}_1^n;\rv{X}_2^n|\rv{W}_{12},\rv{W}_{21},\rv{Y}^n)  - I(\rv{X}_1^n;\rv{Y}^n|\rv{W}_{12},\rv{W}_{21},\rv{X}_2^n) \\
	& = I(\rv{X}_1^n,\rv{X}_2^n;\rv{Y}^n|\rv{W}_{12},\rv{W}_{21}) -I(\rv{X}_2^n;\rv{Y}^n|\rv{W}_{12},\rv{W}_{21},\rv{X}_1^n) \\ 
	&\quad +I(\rv{X}_1^n;\rv{X}_2^n|\rv{W}_{12},\rv{W}_{21},\rv{Y}^n)  - I(\rv{X}_1^n;\rv{Y}^n|\rv{W}_{12},\rv{W}_{21},\rv{X}_2^n) .
\end{align}
Note that
\begin{align}
	I(\rv{X}_2^n;\rv{Y}^n|\rv{W}_{12},\rv{W}_{21},\rv{X}_1^n)
	&= \sum_{i=1}^n I(\rv{X}_2^n;\rv{Y}_i|\rv{W}_{12},\rv{W}_{21},\rv{X}_1^n,\rv{Y}^{i-1}) \\
	&\leq \sum_{i=1}^n I(\rv{X}_{2,i};\rv{Y}_i|\rv{W}_{12},\rv{W}_{21},\rv{X}_{1,i},\rv{Y}^{i-1}) \\
	&= \sum_{i=1}^n I(\rv{X}_{2,i};\rv{Y}_i|\tilde{\rv{U}}_i,\rv{X}_{1,i}) \\
	&=n I(\rv{X}_{2 \rv{Q}};\rv{Y}_{\rv{Q}}|\tilde{\rv{U}}_{\rv{Q}},\rv{X}_{1\rv{Q}},\rv{Q}).
\end{align}
Similarly, one can show that
\begin{equation}
	I(\rv{X}_2^n;\rv{Y}^n|\rv{W}_{12},\rv{W}_{21},\rv{X}_1^n) \leq n I(\rv{X}_{2 \rv{Q}};\rv{Y}_{\rv{Q}}|\tilde{\rv{U}}_{\rv{Q}},\rv{X}_{1\rv{Q}},\rv{Q}).
\end{equation}
Also, we have the following equality
\begin{align}
	I(\rv{X}_1^n,\rv{X}_2^n;\rv{Y}^n|\rv{W}_{12},\rv{W}_{21})
	&= \sum_{i=1}^n I(\rv{X}_1^n,\rv{X}_2^n;\rv{Y}_i|\rv{W}_{12},\rv{W}_{21},\rv{Y}^{i-1}) \\
	&= \sum_{i=1}^n I(\rv{X}_{1,i},\rv{X}_{2,i};\rv{Y}_i|\tilde{\rv{U}}_{i}) \\
	&= n I(\rv{X}_{1\rv{Q}},\rv{X}_{2\rv{Q}};\rv{Y}_{\rv{Q}}|\tilde{\rv{U}}_{\rv{Q}},\rv{Q}).
\end{align}
Combining we obtain the following inequality
\begin{equation}
	\frac{1}{n} I(\rv{W}_{1},\rv{W}_2;\rv{Y}^n)
	\leq C_1+C_2 + I(\rv{X}_{2 \rv{Q}};\rv{Y}_{\rv{Q}}|\tilde{\rv{U}}_{\rv{Q}},\rv{X}_{1\rv{Q}},\rv{Q}) + I(\rv{X}_{2 \rv{Q}};\rv{Y}_{\rv{Q}}|\tilde{\rv{U}}_{\rv{Q}},\rv{X}_{1\rv{Q}},\rv{Q}) - I(\rv{X}_{1\rv{Q}},\rv{X}_{2\rv{Q}};\rv{Y}_{\rv{Q}}|\tilde{\rv{U}}_{\rv{Q}},\rv{Q}).
\end{equation}
Finally, we can also upper bound the rate as follows,
\begin{align}
	I(\rv{M};\rv{Y}^n) 
	&\leq I(\rv{W}_1,\rv{W}_2;\rv{Y}^n)  \\
	&= \sum_{i=1}^n  I(\rv{W}_1,\rv{W}_2;\rv{Y}_i|\rv{Y}^{i-1}) \\
	&\leq \sum_{i=1}^n  I(\rv{X}_{1i},\rv{X}_{2i};\rv{Y}_i) \\
	&= nI(\rv{X}_{1\rv{Q}},\rv{X}_{2Q};\rv{Y}_{\rv{Q}}|\rv{Q}).
\end{align}
The theorem is established after defining the following random variables
\begin{equation}
	\tilde{\rv{U}} \triangleq \tilde{\rv{U}}_{\rv{Q}} \qquad \rv{X}_1 \triangleq \rv{X}_{1\rv{Q}} \qquad \rv{X}_2 \triangleq \rv{X}_{2\rv{Q}} \qquad \rv{Y} \triangleq \rv{Y}_{\rv{Q}}.
\end{equation}


==> sections/upper_bounds_dmc/upper1_bound_proof.tex <==
Consider the first term in the multi-letter upper bound from \autoref{theorem:multiletter_upper_bound} for $ \Omega = \{1,2,3\} $,
%Plugging $ \rv{X} \mapsto \rv{X}_1^n $, $ \rv{Y} \mapsto \rv{X}_2^n $, $ \rv{Z} \mapsto (\rv{W}_{12},\rv{W}_{21}) $  and $ \rv{U} \mapsto \rv{V}^n $ in \autoref{lemma:auxiliary_lemma}, we obtain:
\begin{equation}
	nR \leq n\sum_{\omega \in [3]} C_{\omega, \omega} -  \Gamma(\rv{X}_{[3]}^n|\rv{W}_{c}).
\end{equation}
We apply the methods from \cite{SaeediBidokhti2017} to single-letterize $ \Gamma(\rv{X}_{[3]}^n|\rv{W}_{c}) $ as follows. For any sequence $ \rv{V}^n $
\begin{align}
	&\Gamma(\rv{X}_{[3]}^n|\rv{W}_{c})  \\
	& = \Gamma(\rv{X}_1^n,\rv{X}_2^n,\rv{X}_3^n, \rv{V}^n| \rv{W}_c)  + 2I(\rv{X}_1^n,\rv{X}_2^n,\rv{X}_3^n;\rv{V}^n| \rv{W}_c) \\
	&\minus  I(\rv{V}^n;\rv{X}_1^n,\rv{X}_2^n|\rv{X}_3^n| \rv{W}_c) 
	\minus I(\rv{V}^n;\rv{X}_1^n,\rv{X}_3^n|\rv{X}_2^n| \rv{W}_c) \\
	&\minus I(\rv{V}^n;\rv{X}_2^n,\rv{X}_3^n|\rv{X}_1^n|\rv{W}_c) \\
	&\geq 2 I(\rv{X}_1^n,\rv{X}_2^n,\rv{X}_3^n;\rv{V}^n| \rv{W}_c) \minus I(\rv{V}^n;\rv{X}_1^n,\rv{X}_2^n|\rv{X}_3^n| \rv{W}_c) \\
	& \minus I(\rv{V}^n;\rv{X}_1^n,\rv{X}_3^n|\rv{X}_2^n| \rv{W}_c)
	-I(\rv{V}^n;\rv{X}_2^n,\rv{X}_3^n|\rv{X}_1^n| \rv{W}_c).
\end{align}
Therefore
\begin{multline} \label{eq:multiletter_uppperbound1}
	nR \leq \sum_{\omega \in [3]} C_{\omega \omega} 
	- 2 I(\rv{X}_{[3]}^n;\rv{V}^n| \rv{W}_c) \\
	+ I(\rv{V}^n;\rv{X}_1^n,\rv{X}_2^n|\rv{X}_3^n| \rv{W}_c)
	+I(\rv{V}^n;\rv{X}_1^n,\rv{X}_3^n|\rv{X}_2^n| \rv{W}_c) \\
	+I(\rv{V}^n;\rv{X}_2^n,\rv{X}_3^n|\rv{X}_1^n| \rv{W}_c)
\end{multline}
The most challenging term here is
$ 	- 2 I(\rv{X}_{[3]}^n;\rv{V}^n| \rv{W}_c)  $.
Consider the following cut-set bound on $ R $.
\begin{multline}\label{eq:multiletter_uppperbound2}
	nR \leq    n \sum_{\omega \in [3]}  \sum_{\omega' \neq \omega} C_{\omega,\omega'} +   I(\rv{X}_{[3]}^n;\rv{Y}^n|\rv{W}_c)  \\
	\leq n \sum_{\omega \in [3]}  \sum_{\omega' \neq \omega} C_{\omega,\omega'} +   I(\rv{X}_{[3]}^n, ;\rv{Y}^n, \rv{V}^n|\rv{W}_c) .
\end{multline}
Combining \eqref{eq:multiletter_uppperbound1} and two times \eqref{eq:multiletter_uppperbound2} we obtain
\begin{multline}\label{eq:multiletter_uppperbound3}
	3nR \leq n \sum_{\omega \in [3]} C_{\omega \omega }  +  2 n \sum_{\omega \in [3]}  \sum_{\omega' \neq \omega} C_{\omega,\omega'} \\
	+2I(\rv{X}_{[3]}^n;\rv{Y}^n|\rv{W}_c,\rv{V}^n) 
	+ I(\rv{V}^n;\rv{X}_1^n,\rv{X}_2^n|\rv{W}_c,\rv{X}_3^n) \\
	+I(\rv{V}^n;\rv{X}_1^n,\rv{X}_3^n|\rv{W}_c,\rv{X}_2^n) 
	+I(\rv{V}^n;\rv{X}_2^n,\rv{X}_3^n|\rv{W}_c,\rv{X}_1^n).
\end{multline}
We now choose $ \rv{V}_i $, $ i=1,\dots,n $, to be the output of a memoryless channel $ \mathsf{P}_{\rv{V}|\rv{X}_{[3]} \rv{Y}}(v_i|x_{[3]i},y_i) $ with input $ (\rv{X}_{[3]i},\rv{Y}_i) $. 
As was suggested in \cite{Wigger2008}, we introduce $ \tilde{\rv{U}}_i \triangleq (\rv{W}_{c}) $.  
Furthermore, let $ \rv{Q} $ be a uniform random variable over $ [n] $. With this choice we obtain the following list of inequalities:
\begin{align}
	I(\rv{X}_1^n,\rv{X}_2^n,\rv{X}_3^n;\rv{Y}^n|\rv{W}_c,\rv{V}^n)
	&= \sum_{i=1}^n I(\rv{X}_1^n,\rv{X}_2^n,\rv{X}_3^n;\rv{Y}_i|\rv{W}_c,\rv{V}^n, \rv{Y}^{i-1})  \\
	&\eqann{\leq}{a} \sum_{i=1}^n I(\rv{X}_{1i},\rv{X}_{2i},\rv{X}_{3i};\rv{Y}_i|\rv{U}_i,\rv{V}_i) \\
	& = n   I(\rv{X}_{1\rv{Q}},\rv{X}_{2\rv{Q}},\rv{X}_{3\rv{Q}};\rv{Y}_{\rv{Q}}|\rv{U}_{\rv{Q}},\rv{V}_{\rv{Q}},\rv{Q} ) \\
	&\eqann{=}{b} n   I(\rv{X}_{1},\rv{X}_{2},\rv{X}_{3};\rv{Y}|\tilde{\rv{U}},\rv{V},\rv{Q}),
\end{align}
where \eqannref{a}  follows due to the Markov chain
\begin{equation} \label{eq:markov_chain_UX1X2X3Y}
	(\rv{X}_1^n,\rv{X}_2^n,\rv{X}_3^n,\rv{U}^n,\rv{Y}^{i-1}) \rightarrow
	(\rv{X}_{1i},\rv{X}_{2i},\rv{X}_{3i},\rv{U}_{i}) \rightarrow \rv{Y}_i.
\end{equation}
and in \eqannref{b} we defined the following random variables:
\begin{equation}
	\rv{X}_{k} \triangleq \rv{X}_{k,\rv{Q}} \forall k \in \{1,2,3\}, \quad \rv{Y} \triangleq  \rv{Y}_{\rv{Q}}, \quad  \rv{U} \triangleq \rv{U}_{\rv{Q}}.
\end{equation}
In a very similar manner we single-letterize the remaining terms in \eqref{eq:multiletter_uppperbound3}
\begin{align}
	I(\rv{V}^n;\rv{X}_1^n,\rv{X}_2^n|\rv{W}_c,\rv{X}_3^n) 
	&= \sum_{i=1}^{n} I(\rv{V}_i;\rv{X}_1^n,\rv{X}_2^n|\rv{W}_c,\rv{X}_3^n, \rv{V}^{i-1}) \\
	&\eqann{\leq}{a} \sum_{i=1}^{n} I(\rv{V}_i;\rv{X}_{1i},\rv{X}_{2i}|\tilde{\rv{U}}_i,\rv{X}_{3i}) \\
	&= n  I(\rv{V}_{\rv{Q}};\rv{X}_{1\rv{Q}},\rv{X}_{2\rv{Q}}|\tilde{\rv{U}}_{\rv{Q}},\rv{X}_{3\rv{Q}},\rv{Q}) \\
	&= n  I(\rv{V};\rv{X}_{1},\rv{X}_{2}|\tilde{\rv{U}},\rv{X}_{3},\rv{Q})
\end{align}
where \eqannref{a}  follows due to the Markov chain
\begin{equation} \label{eq:mzrkov_chain_X1X2X3U}
	(\rv{X}_1^n,\rv{X}_2^n,\rv{X}_3^n,\rv{V}^{i-1}) \rightarrow
	(\rv{X}_{1i},\rv{X}_{2i},\rv{X}_{3i}) \rightarrow \rv{V}_i.
\end{equation}
Similarly, one can show that
\begin{align}
	I(\rv{V}^n;\rv{X}_1^n,\rv{X}_3^n|\rv{W}_c,\rv{X}_2^n) 
	&\leq n  I(\rv{V};\rv{X}_{1},\rv{X}_{3}|\tilde{\rv{U}},\rv{X}_{2},\rv{Q}) \\
	I(\rv{V}^n;\rv{X}_2^n,\rv{X}_3^n|\rv{W}_c,\rv{X}_1^n) 
	&\leq n  I(\rv{V};\rv{X}_{2},\rv{X}_{3}|\tilde{\rv{U}},\rv{X}_{1},\rv{Q}).
\end{align}

%\begin{align}
%	I(\rv{X}_1^n;\rv{X}_2^n|\rv{X}_3^n) 
%	& = I(\rv{X}_1^n,\rv{U}^n;\rv{X}_2^n|\rv{X}_3^n) 
%	- I(\rv{U}^n;\rv{X}_2^n|\rv{X}_1^n,\rv{X}_3^n) \\
%	& = I(\rv{U}^n;\rv{X}_2^n|\rv{X}_3^n) 
%	+ I(\rv{X}_1^n;\rv{X}_2^n|\rv{U}^n,\rv{X}_3^n) 
%	- I(\rv{U}^n;\rv{X}_2^n|\rv{X}_1^n,\rv{X}_3^n) \\
%	& = I(\rv{U}^n;\rv{X}_1^n,\rv{X}_2^n|\rv{X}_3^n) 
%	- I(\rv{U}^n;\rv{X}_1^n|\rv{X}_2^n,\rv{X}_3^n) 
%	+ I(\rv{X}_1^n;\rv{X}_2^n|\rv{U}^n,\rv{X}_3^n) 
%	- I(\rv{U}^n;\rv{X}_2^n|\rv{X}_1^n,\rv{X}_3^n) \\
%	&\geq I(\rv{U}^n;\rv{X}_1^n,\rv{X}_2^n|\rv{X}_3^n) 
%	- I(\rv{U}^n;\rv{X}_1^n|\rv{X}_2^n,\rv{X}_3^n) 
%	- I(\rv{U}^n;\rv{X}_2^n|\rv{X}_1^n,\rv{X}_3^n) 
%\end{align}
%
%Therefore
%\begin{equation} \label{eq:multiletter_uppperbound4}
%	nR \leq \sum_{i,j=1}^{3} C_{ij} 
%	-  I(\rv{X}_1^n,\rv{X}_2^n;\rv{U}_n|\rv{X}_3^n) 
%	+ I(\rv{U}^n;\rv{X}_1^n|\rv{X}_2^n,\rv{X}_3^n)
%	+I(\rv{U}^n;\rv{X}_2^n|\rv{X}_1^n,\rv{X}_3^n)
%\end{equation}
%We would like to eliminate the term
%\begin{equation}
%	-  I(\rv{X}_1^n,\rv{X}_2^n;\rv{U}_n|\rv{X}_3^n) .
%\end{equation}
%Consider the \acrshort{mac} cut-set bound on $ R $.
%\begin{equation}\label{eq:multiletter_uppperbound5}
%	nR \leq C_{33} +  I(\rv{X}_1^n,\rv{X}_2^n;\rv{Y}^n|\rv{X}_3^n)
%	\leq C_3 + I(\rv{X}_1^n,\rv{X}_2^n;\rv{Y}^n,\rv{U}^n|\rv{X}_3^n).
%\end{equation}
%Combining \eqref{eq:multiletter_uppperbound4} and  \eqref{eq:multiletter_uppperbound5} we obtain
%\begin{equation}\label{eq:multiletter_uppperbound6}
%	2nR \leq \sum_{i,j=1}^{3} C_{ij} 
%	+I(\rv{X}_1^n,\rv{X}_2^n;\rv{Y}^n|\rv{U}^n,\rv{X}_3^n)
%	+ I(\rv{U}^n;\rv{X}_1^n|\rv{X}_2^n,\rv{X}_3^n)
%	+I(\rv{U}^n;\rv{X}_2^n|\rv{X}_1^n,\rv{X}_3^n).
%\end{equation}
%Considering each of the terms in \eqref{eq:multiletter_uppperbound6} we obtain
%\begin{align}
%	I(\rv{X}_1^n,\rv{X}_2^n;\rv{Y}^n|\rv{U}^n,\rv{X}_3^n)
%	&= \sum_{i=1}^n I(\rv{X}_1^n,\rv{X}_2^n;\rv{Y}_i|\rv{U}^n,\rv{X}_3^n, \rv{Y}^{i-1})  \\
%	&\eqann{\leq}{a} \sum_{i=1}^n I(\rv{X}_{1i},\rv{X}_{2i};\rv{Y}_i|\rv{U}_i,\rv{X}_{3i}) \\
%	& = n   I(\rv{X}_{1\rv{Q}},\rv{X}_{2\rv{Q}};\rv{Y}_{\rv{Q}}|\rv{U}_{\rv{Q}} ,\rv{X}_{3\rv{Q}},\rv{Q}) \\
%	&= n   I(\rv{X}_{1},\rv{X}_{2};\rv{Y}|\rv{U},\rv{X}_{3},\rv{Q}),
%\end{align}
%where \eqannref{a}  follows due to the Markov chain (which is identical to \eqref{eq:markov_chain_UX1X2X3Y} )
%\begin{equation}
%	(\rv{X}_1^n,\rv{X}_2^n,\rv{X}_3^n,\rv{U}^n,\rv{Y}^{i-1}) \rightarrow
%	(\rv{X}_{1i},\rv{X}_{2i},\rv{X}_{3i},\rv{U}_{i}) \rightarrow \rv{Y}_i.
%\end{equation}
%In a very similar manner we single-letterize the remaining terms in \eqref{eq:multiletter_uppperbound6}
%\begin{align}
%	I(\rv{U}^n;\rv{X}_1^n|\rv{X}_2^n,\rv{X}_3^n) 
%	&= \sum_{i=1}^{n} I(\rv{U}_i;\rv{X}_1^n|\rv{X}_2^n,\rv{X}_3^n, \rv{U}^{i-1}) \\
%	&\eqann{\leq}{a} \sum_{i=1}^{n} I(\rv{U}_i;\rv{X}_{1i}|\rv{X}_{2i},\rv{X}_{3i}) \\
%	&= n  I(\rv{U}_{\rv{Q}};\rv{X}_{1\rv{Q}}|\rv{X}_{2\rv{Q}},\rv{X}_{3\rv{Q}},\rv{Q}) \\
%	&\leq n  I(\rv{U}_{\rv{Q}};\rv{X}_{1\rv{Q}}|\rv{X}_{2\rv{Q}},\rv{X}_{3\rv{Q}}, \rv{Q}) \\
%	&= n  I(\rv{U};\rv{X}_{1}|\rv{X}_{2},\rv{X}_{3}, \rv{Q})
%\end{align}
%where \eqannref{a}  follows due to the Markov chain (which is identical to \eqref{eq:mzrkov_chain_X1X2X3U})
%\begin{equation}
%	(\rv{X}_1^n,\rv{X}_2^n,\rv{X}_3^n,\rv{U}^{i-1}) \rightarrow
%	(\rv{X}_{1i},\rv{X}_{2i},\rv{X}_{3i}) \rightarrow \rv{U}_i.
%\end{equation}
%Similarly,
%\begin{equation}
%	I(\rv{U}^n;\rv{X}_2^n|\rv{X}_1^n,\rv{X}_3^n) 
%	\leq n  I(\rv{U};\rv{X}_{2}|\rv{X}_{1},\rv{X}_{3}).
%\end{equation}
%
%
%In a very similar fashion,  we can obtain:
%\begin{equation}
%	nR
%	= C_{11}+C_{12}+C_{13} +  I(\rv{X}_2^n,\rv{X}_3^n;\rv{Y}^n|\rv{X}_1^n) + n \epsilon_n ,
%\end{equation}
%with
%\begin{align}
%	I(\rv{X}_2^n,\rv{X}_3^n;\rv{Y}^n|\rv{X}_1^n) 
%	&= \sum_{i=1}^n I(\rv{X}_2^n,\rv{X}_3^n;\rv{Y}_i|\rv{X}_1^n,\rv{Y}^{i-1}) \\
%	&= \sum_{i=1}^n H(\rv{Y}_i|\rv{X}_1^n,\rv{Y}^{i-1}) - \sum_{i=1}^n H(\rv{Y}_i|\rv{X}_1^n,\rv{X}_2^n,\rv{X}_3^n,\rv{Y}^{i-1}) \\
%	&= \sum_{i=1}^n H(\rv{Y}_i|\rv{X}_1^n,\rv{Y}^{i-1},\rv{U}^{i-1}) - \sum_{i=1}^n H(\rv{Y}_i|\rv{X}_1^n,\rv{X}_2^n,\rv{X}_3^n,\rv{Y}^{i-1},\rv{U}^{i-1}) \\
%	&\leq \sum_{i=1}^n H(\rv{Y}_i|\rv{X}_{1,i},\rv{U}^{i-1}) - \sum_{i=1}^n H(\rv{Y}_i|\rv{X}_{1,i},\rv{X}_{2,i},\rv{X}_{3,i},\rv{U}^{i-1}) \\
%	&= n H(\rv{Y}_{\rv{T}}|\rv{X}_{1,\rv{T}},\rv{U}^{\rv{T}-1},\rv{T}) - n H(\rv{Y}_\rv{T}|\rv{X}_{1,\rv{T}},\rv{X}_{2,\rv{T}},\rv{X}_{3,\rv{T}},\rv{U}^{\rv{T}-1},\rv{T}) \\
%	&= I(\rv{X}_{2},\rv{X}_3;\rv{Y}|\rv{X}_1,\rv{Q}).
%\end{align}
%The other inequalities follow in similar manner.






As for \eqref{eq:multiletter_upper_bound3}, we have
\begin{align*}
	I(\rv{X}_{\set{S}^c}^n;\rv{Y}^n|\rv{W}_c,\rv{X}_{\set{S}}^n)
	&= \sum_{i=1}^n I(\rv{X}_{\set{S}^c}^n;\rv{Y}_i|\rv{W}_{c},\rv{X}_{\set{S}}^n,\rv{Y}^{i-1}) \\
	&\leq \sum_{i=1}^n I(\rv{X}_{\set{S}^c,i};\rv{Y}_i|\tilde{\rv{U}}_{i},\rv{X}_{\set{S},i}) \\
	&=  n I(\rv{X}_{\set{S}^c\rv{Q}};\rv{Y}_{\rv{Q}}| \tilde{\rv{U}}_{\rv{Q}}, \rv{X}_{\set{S}\rv{Q}},\rv{Q}) \\
	&=  n I(\rv{X}_{\set{S}^c};\rv{Y}|\tilde{\rv{U}},\rv{X}_{\set{S}},\rv{Q}).
\end{align*}
In a very similar manner, one can show that
\begin{equation}
	I(\rv{X}_{\Omega};\rv{Y}^n) \leq n I(\rv{X}_{\Omega};\rv{Y}|\rv{Q}).
\end{equation}
 Furthermore, since
\begin{equation}
	I(\rv{X}_{\Omega};\rv{Y}|\rv{Q})  \leq I(\rv{X}_{\Omega},\rv{Q};\rv{Y}) = I(\rv{X}_{\Omega};\rv{Y})   ,
\end{equation}
and identifying $ \rv{U} \triangleq (\tilde{\rv{U}}, \rv{Q}) $, we obtain the proof of the theorem.

